Selection of Prompt Engineering Techniques for Code Generation through Predicting Code Complexity

Large Language Models (LLMs) have demonstrated impressive performance in software engineering tasks. However, improving their accuracy in generating correct and reliable code remains challenging. Numerous prompt engineering techniques (PETs) have been developed to address this, but no single approach is universally optimal. Selecting the right PET for each query is difficult for two primary reasons: (1) interactive prompting techniques may not consistently deliver the expected benefits, especially for simpler queries, and (2) current automated prompt engineering methods lack adaptability and fail to fully utilize multi-stage responses. To overcome these challenges, we propose PET-Select, a PET-agnostic selection model that uses code complexity as a proxy to classify queries and select the most appropriate PET. By incorporating contrastive learning, PET-Select effectively distinguishes between simple and complex problems, allowing it to choose PETs that are best suited for each query's complexity level. Our evaluations on the MBPP and HumanEval benchmarks using GPT-3.5 Turbo and GPT-4o show up to a 1.9% improvement in pass@1 accuracy, along with a 74.8% reduction in token usage. Additionally, we provide both quantitative and qualitative results to demonstrate how PET-Select effectively selects the most appropriate techniques for each code generation query, further showcasing its efficiency in optimizing PET selection.

==> pics/HumanEval_distribution.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            symbolic x coords={Algorithm Design, String Manipulation, List Processing, Mathematical Computation, Parsing and Formatting, Logical Conditions},
            xtick=data,
            ymin=0,
            ymax=50,
            ylabel={Correct Instances},
            xlabel={Tasks},
            bar width=0.1cm, % Adjust the bar width to fit more bars
            nodes near coords,
            nodes near coords style={
                font=\fontsize{5pt}{4pt}\selectfont % This changes the font size to small
            },
            enlarge x limits={abs=1.1cm}, % Enlarges the x-axis to fit the bars better
            legend style={anchor=north east, legend cell align={left}, font=\tiny}, 
            width = \linewidth,
            height = 0.5\linewidth,
            tick label style={font=\fontsize{5pt}{5pt}\selectfont},
            ylabel near ticks,
        ]
            \addplot+[bar shift=-0.8cm, fill=blue!30, draw=blue!80, text=blue!80] coordinates {(Algorithm Design,13) (String Manipulation,34) (List Processing,43) (Mathematical Computation,35) (Parsing and Formatting,5) (Logical Conditions, 1)};
            \addplot+[bar shift=-0.6cm, fill=blue!70, draw=blue!100, text=blue!100] coordinates {(Algorithm Design,12) (String Manipulation,38) (List Processing,46) (Mathematical Computation,35) (Parsing and Formatting,5) (Logical Conditions, 1)};
            \addplot+[bar shift=-0.4cm, fill=red!30, draw=red!80, text=red!80] coordinates {(Algorithm Design,12) (String Manipulation,36) (List Processing,42) (Mathematical Computation,34) (Parsing and Formatting,5) (Logical Conditions, 2)};
            \addplot+[bar shift=-0.2cm, fill=red!70, draw=red!100, text=red!100] coordinates {(Algorithm Design,13) (String Manipulation,40) (List Processing,44) (Mathematical Computation,34) (Parsing and Formatting,4) (Logical Conditions, 2)};
            \addplot+[bar shift=0cm, fill=brown!50, draw=brown!100, text=brown!100] coordinates {(Algorithm Design,13) (String Manipulation,37) (List Processing,42) (Mathematical Computation,32) (Parsing and Formatting,4) (Logical Conditions, 1)};
            \addplot+[bar shift=0.2cm, fill=teal!50, draw=teal!100, text=teal!100] coordinates {(Algorithm Design,10) (String Manipulation,32) (List Processing,41) (Mathematical Computation,32) (Parsing and Formatting,4) (Logical Conditions, 1)};
            \addplot+[bar shift=0.4cm, fill=black!50, draw=black!100, text=black!100] coordinates {(Algorithm Design,9) (String Manipulation,21) (List Processing,26) (Mathematical Computation,28) (Parsing and Formatting,5) (Logical Conditions, 1)};
            \addplot+[bar shift=0.6cm, fill=violet, draw=violet, text=violet] coordinates {(Algorithm Design,15) (String Manipulation,35) (List Processing,37) (Mathematical Computation,34) (Parsing and Formatting,5) (Logical Conditions, 1)};
            \addplot+[bar shift=0.8cm, fill=olive, draw=olive, text=olive] coordinates {(Algorithm Design,13) (String Manipulation,38) (List Processing,45) (Mathematical Computation,34) (Parsing and Formatting,5) (Logical Conditions, 1)};
            
            \legend{Zero-shot, Zero-shot CoT, Few-shot, Few-shot CoT, Self-debug, Self-plan, Reflection, Progressive Hint, Persona} % Adds a legend
        \end{axis}
    \end{tikzpicture}
    \caption{HumanEval on GPT-4o}
    \label{HumanEval_distribution}
\end{figure}

==> pics/MBPP_complexity.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            ybar,
            symbolic x coords={Line Complexity, Cyclomatic Complexity, Halstead Metric, Cognition Complexity, Maintainability Index, Combined Complexity},
            xtick=data,
            ymin=0,
            ymax=105,
            ylabel={Values},
            xlabel={Code Complexity Metrics},
            bar width=0.1cm, % Adjust the bar width to fit more bars
            nodes near coords,
            nodes near coords style={
                font=\fontsize{3.5pt}{3pt}\selectfont % This changes the font size to small
            },
            enlarge x limits={abs=1.1cm}, % Enlarges the x-axis to fit the bars better
            % legend style={anchor=north east, legend cell align={left}, font=\tiny}, 
            legend style={
                at={(0.05,0.95)}, % Moves the legend to the upper left
                anchor=north west, % Anchors the legend at the north west
                legend cell align={left},
                font=\tiny
            },
            width = \linewidth,
            height = 0.5\linewidth,
            tick label style={font=\fontsize{5pt}{5pt}\selectfont},
            ylabel near ticks,
        ]
            \addplot+[bar shift=-0.8cm, fill=blue!30, draw=blue!80, text=blue!80] coordinates {(Line Complexity,5.9) (Cyclomatic Complexity,2.6) (Halstead Metric,6.7) (Cognition Complexity,2.1) (Maintainability Index,79.3) (Combined Complexity, 96.6)};
            
            \addplot+[bar shift=-0.6cm, fill=blue!70, draw=blue!100, text=blue!100] coordinates {(Line Complexity,7.5) (Cyclomatic Complexity,3.6) (Halstead Metric,9.2) (Cognition Complexity,3.2) (Maintainability Index,74.9) (Combined Complexity, 98.5)};
            
            \addplot+[bar shift=-0.4cm, fill=red!30, draw=red!80, text=red!80] coordinates {(Line Complexity,7.5) (Cyclomatic Complexity,3.4) (Halstead Metric,8.2) (Cognition Complexity,3.1) (Maintainability Index,75.0) (Combined Complexity, 97.2)};
            
            \addplot+[bar shift=-0.2cm, fill=red!70, draw=red!100, text=red!100] coordinates {(Line Complexity,5.3) (Cyclomatic Complexity,3.0) (Halstead Metric,7.4) (Cognition Complexity,2.6) (Maintainability Index,77.7) (Combined Complexity, 96.0)};
            
            \addplot+[bar shift=0cm, fill=brown!50, draw=brown!100, text=brown!100] coordinates {(Line Complexity,6.6) (Cyclomatic Complexity,2.6) (Halstead Metric,5.6) (Cognition Complexity,1.5) (Maintainability Index,82.8) (Combined Complexity, 99.2)};
            
            \addplot+[bar shift=0.2cm, fill=teal!50, draw=teal!100, text=teal!100] coordinates {(Line Complexity,7) (Cyclomatic Complexity,2.6) (Halstead Metric,6.8) (Cognition Complexity,2.6) (Maintainability Index,78.9) (Combined Complexity, 97.9)};
            
            \addplot+[bar shift=0.4cm, fill=black!50, draw=black!100, text=black!100] coordinates {(Line Complexity,7.3) (Cyclomatic Complexity,3.4) (Halstead Metric,9.3) (Cognition Complexity,3.5) (Maintainability Index,75.0) (Combined Complexity, 98.5)};
            
            \addplot+[bar shift=0.6cm, fill=violet, draw=violet, text=violet] coordinates {(Line Complexity,6.0) (Cyclomatic Complexity,4.0) (Halstead Metric,6.8) (Cognition Complexity,2.3) (Maintainability Index,79.7) (Combined Complexity, 98.7)};
            
            \addplot+[bar shift=0.8cm, fill=olive, draw=olive, text=olive] coordinates {(Line Complexity,9.0) (Cyclomatic Complexity,4.0) (Halstead Metric,11.5) (Cognition Complexity,3.9) (Maintainability Index,69.1) (Combined Complexity, 97.5)};
            
            \legend{Zero-shot, Zero-shot CoT, Few-shot, Few-shot CoT, Self-debug, Self-plan, Reflection, Progressive Hint, Persona} % Adds a legend
        \end{axis}
    \end{tikzpicture}
    \caption{MBPP on GPT-3.5 Turbo}
    \label{MBPP_complexity}
\end{figure}

==> tabs/RQ3_metrics.tex <==

\begin{table}
    \centering
    \caption{MRR and nDCG metrics on the test set using \tool.}
    \label{tab:metrics}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{lrr}
    \toprule
         &  MRR& nDCG@9\\
    \midrule
         MBPP on GPT-3.5 Turbo&     0.5166&  0.6948\\
         MBPP on GPT-4o&  0.5648& 0.6840\\
         HumanEval on GPT-3.5 Turbo&  0.6186& 0.7270\\
         HumanEval on GPT-4o&  0.6027& 0.8269\\
    \bottomrule
    \end{tabular}
    }
    
\end{table}
